The Life and Death of SSDs and HDDs: Similarities, Differences, and Prediction Models

Data center downtime typically centers around IT equipment failure. Storage devices are the most frequently failing components in data centers. We present a comparative study of hard disk drives (HDDs) and solid state drives (SSDs) that constitute the typical storage in data centers. Using a six-year field data of 100,000 HDDs of different models from the same manufacturer from the BackBlaze dataset and a six-year field data of 30,000 SSDs of three models from a Google data center, we characterize the workload conditions that lead to failures and illustrate that their root causes differ from common expectation but remain difficult to discern. For the case of HDDs we observe that young and old drives do not present many differences in their failures. Instead, failures may be distinguished by discriminating drives based on the time spent for head positioning. For SSDs, we observe high levels of infant mortality and characterize the differences between infant and non-infant failures. We develop several machine learning failure prediction models that are shown to be surprisingly accurate, achieving high recall and low false positive rates. These models are used beyond simple prediction as they aid us to untangle the complex interaction of workload characteristics that lead to failures and identify failure root causes from monitored symptoms.

==> SC19.tex <==


% \newcommand{\makeimage}[1]{%
% \begin{center} 	\includegraphics[width=0.9\linewidth]{#1} \end{center}
% }

\section{Introduction}

% Outline: (1) what are we studying and why? (SSD reliability, failure characteristics); (2) what is our methodology? (3) what do we find?

% {\bf E2J: seems to me that failures and retirements are used incorectly -- can you please make a careful pass through the introduction to fix this?}


The longevity of solid state drives (SSDs) and their reliability is of much importance in recent years as increasing amounts of data in modern data centers reside on SSDs.
Unfortunately, there are relatively few studies on the reliability of SSD devices, especially compared to the extensive studies of hard disk drives (HDDs) occurring over the past several decades. HDD reliability research is not generalizable to SSDs as
the physical mechanics of HDDs are distinct from SSDs and, correspondingly, their failure symptoms and causes are fundamentally different.
For the few existing SSD reliability analyses, their scope has focused more on specific errors in controlled, laboratory environments using simulated workloads~\cite{DBLP:conf/sigmetrics/LuoGCHM18,DBLP:conf/hpca/CaiLHMM15,DBLP:conf/dsn/QureshiKKNM15,DBLP:conf/micro/GruppCCSYSW09,DBLP:conf/fast/ZhengTQL13}.
Non-simulated studies of SSD reliability analysis, centered around production systems, typically focus on the type of errors (in particular, raw bit error rates and uncorrectable bit error rates), their relationship with the workload, drive age, and drive wear out. However these results also extend to field characteristics of block failures, chip failures, and rates of repairs and replacements~\cite{BiancaFAST16,mahdisoltani2017proactive,MezaWKM15}.

%The above study concluded that raw bit errors, the standard metric for drive reliability, are not good predictors of uncorrectable bit error rates or failures that a a major concern in practice. 
%Since there is no clear culprit that leads to identification of uncorrectable errors, the authors in~\cite{mahdisoltani2017proactive} resort to machine learning prediction models and find that random forest models offer good accuracy for engaging proactive techniques such adaptive the disk scrubbing speed.

In this paper we look into the process of SSD retirements by examining those drive failures that necessitate manual intervention and repairs. We study this through analysis of a selection of daily performance logs for three multi-level cell (MLC) models collected at a Google production data center over the course of six years.
We concern ourselves with the conditions of drive activity that precede these total failures. 
% It is obvious that the presence of hardware errors portends drive failure, but the precise conditions that trigger these failures remain unclear.
Though we are unaware of the data center's exact workflow for drive repairs and replacements (e.g., whether they are done manually or automatically, or the replacement policies in place), we are able to discover key correlations and patterns of failure, as well as generate useful forecasts of future failures.
%, after certain performance or reliability thresholds are crossed,
% or what is the entirety of conditions that lead to a retirement.
Being able to predict an upcoming retirement could allow early action: for example,
early replacement before failure happens, migration of data and VMs to other resources, or even allocation of VMs to disks that are not prone to failure~\cite{XuATC18}.


In this paper, we study the various error types accounted by the logs to determine their roles in triggering, or otherwise portending, future drive failures.
It is interesting to note that although we have ample data, statistical methods are not able to achieve highly accurate predictions: we find no evidence that the repair process is triggered by any deterministic decision rule. 
%This fact indicates that randomness has a large part to play in drive failures.
%We resort employ machine learning, aiming  a better understanding of the causes preceding drive failures.
Since the complexity of the data does not allow for a typical treatment of prediction based on straightforward statistical analysis, we resort to machine learning predictors to help us detect which quantitative measures provide strong indications of upcoming failures.
We show that machine learning models that are trained from SSD monitoring logs achieve failure prediction that is both
remarkably accurate and timely. 
% The models confirm that drive replacements are not triggered by na\"\i{}ve thresholding of predictors. 
Beyond prediction, the models are interpreted to provide valuable insights on which errors and workload characteristics are most indicative of future catastrophic failures.

The models are able to anticipate failure events with reasonable accuracy up to several days in advance, despite some inherent methodological challenges. Although the frequency of failures is significant (14\% of the drives experience failures during their lifetime), the data set is highly imbalanced. % containing 1 failure case for each 10,000 non-failure cases. 
This is a common problem in classification, and makes achieving simultaneously high true positive rates and low false positive ones very difficult. 
We train a set of six machine learning predictors and illustrate that it is possible to achieve robust predictions.
Crucially, we focus on the interpretability of the machine learning models and derive insights 
% that can be used for timely prediction of upcoming failures 
that can be used to drive proactive SSD management policies.
%Accordingly, we choose to measure performance using the receiver operating characteristic (ROC) curve, which is insensitive to class imbalance and illustrates the diagnostic performance of a binary classifier system as its discrimination threshold is varied.
%The ROC AUC metric (area under the curve) is used to assess prediction performance~\cite{FAWCETT2006861}
%We observe that many of these drive repairs tend to occur after a period of several days in which the affected drive appears to have entirely ceased to function. Furthermore, after the repair process has terminated, many drives do not re-enter the fleet; if they do, it is often not until several months to years after their dismissal. It is interesting to note that roughly half of repairs are not observed to terminate; in such a case, it is likely that the drive is deemed retired.
Our findings are summarized as follows:
%We observe that many of these drive repairs tend to occur after a period of several days in which the affected drive appears to have entirely ceased to function. Furthermore, after the repair process has terminated, many drives do not re-enter the fleet; if they do, it is often not until several months to years after their dismissal. It is interesting to note that roughly half of repairs are not observed to terminate; in such a case, it is likely that the drive is deemed retired.
% \vspace*{-0.2cm}
\begin{itemize}[leftmargin=*]
\item Although a significant portion of drives (up to 14\%) are swapped during their lifetime, a very small percentage of swapped drives that go into repair mode re-enter the workflow within a month, this percentage is as low as 5\% and as high as 9.4\%, depending on the drive type. Up to 28\% of drives are repaired within a year and about 50\% of those that are swapped are never put back into production.
\item A significant proportion of failed drives (roughly 10\%) remain in the system in a failed state for a period on the order of months.
\item There is no single metric that triggers a drive failure after it reaches a certain threshold.
\item Several different machine learning predictors are quite successful for failure prediction. Random forests are found to be the most successful of all.
\item We identify the drive age as the most important feature for swap prediction (and also for non-transparent error prediction).
\item \newtext{We are unable to demonstrate a correspondence between P/E cycles and failure, suggesting that write behavior is not as highly indicative of failure as previously thought.}
\item Different predictors need to be trained for drives of different age groups and the which features are useful for failure prediction depends heavily on the age of the drive.
\end{itemize}
The above insights can be used to anticipate failures and take appropriate actions such as proactive SSD management, spare drive provisioning, and perhaps even workload allocation. 

This paper is organized as follows. We first characterize the data and summarize our findings in Section~\ref{sec:SSDtraceErrorLog} and~\ref{sec:SSDtraceSwapLog}, respectively. Section~\ref{sec:data}  connects statistics between failure statistics to workload statistics to identify symptoms and causes of drive failures.
In Section~\ref{sec:ML}, we propose several machine learning predictors of SSD failure and conduct detailed post-prediction analysis. Section~\ref{SEC:related} presents related work, followed by the summary and conclusions in Section~\ref{sec:conclusion}.

\section{SSD Trace Data}
\label{sec:SSDtraceErrorLog}
The data consist of daily performance logs for three MLC SSD models collected at a Google data center over a period of six years. Each of the three models are  manufactured by the same vendor and have a capacity 480GB and a lithography on the order of 50nm. All three models utilize custom firmware and drivers, meaning that error reporting is done in a proprietary format rather than through standard SMART features~\cite{SMART}.  We refer to the three models as MLC-A, MLC-B, and MLC-D in accordance with the naming in~\cite{BiancaFAST16,mahdisoltani2017proactive}. We have data on over 10,000 unique drives for each drive model, totaling over 40,000,000 daily drive reports overall.

% \begin{table*}
% 	\centering
%   \begin{tabular}{|c|c|c|c|c|} \hline
%   SSD Model & \#Drives & Capacity & Lithography (nm) & P/E cycle limit \\ \hline \hline
%   MLC-A & 10181 & 480GB & 50 & 3,000 \\ \hline
%   MLC-B & 10200 & 480GB & 43 & 3,000 \\ \hline
%   MLC-D & 10359 & 480GB & 50 & 3,000 \\ \hline
%   \end{tabular}
%   \caption{Drive model statistics (taken from [Bianca ATC])}
%   \label{table:models}
% \end{table*}

% {\bf E: how many entries? Granularity? More high level info for the log?.}

% \remove{In this paper, we reference two different logs. The first of these is the {\em error log}, which holds the daily summaries of drive activity. For each day of each drive's activity, the error log reports each of the following metrics:}
{The logs used in this paper report daily summaries of drive activity. Drives are uniquely identified by their drive ID, which is a hashed value of their serial number. For each day of operation, the following metrics are reported:}
\begin{itemize}[leftmargin=*]
% 	\item The drive's model and ID number
    \item The timestamp of the report, given in microseconds since the beginning of the drive's lifetime
    \item The number of read, write, and erase operations performed by the drive over the course of the day
    \item The cumulative number of program--erase (P/E) cycles seen by the drive over its lifetime. A program--erase cycle is the process by which a memory cell is written to and subsequently erased. The cumulative amount of these cycles is a measure of device wear.
    \item Two status flags indicating whether the drive has died and whether the drive is operating in read-only mode. 
    \item The number of {\em bad blocks} in the drive. A block is marked bad either when it is non-operational upon purchase (denoted a {\em factory bad block}) or when a non-transparent error occurs in the block and it is subsequently removed from use. Cumulative counts of both of these bad block types are provided in the log.
    \item The counts of different errors that have occurred over the course of the day, specific counts are provided for the following error types:
    \begin{itemize}
    	\item {\em correctable error}: the total number of bits that were found corrupted and corrected using drive-internal error correction codes (ECC) during read operations during that day,
        \item {\em erase error}: number of erase operations that failed, 
        \item {\em final read error}: the number of read operations that fail, even after (drive-initiated) retries, 
        \item {\em final write error}: the number of write operations that fail, even after (drive-initiated) retries,
        \item {\em meta error}: number of errors encountered while reading drive-internal metadata,
        \item {\em read error}: the number of read operations that experienced an error, but succeeded on retry (initiated drive-internally),
        \item {\em response error}: number of bad responses from the drive,
        \item {\em timeout error}: number of operations that timed out after some wait period,
        \item {\em uncorrectable error}: number of uncorrectable ECC errors encountered during read operations during that day, and
        \item {\em write error}: the number of write operations that experienced an error, but succeeded on retry (initiated drive-internally).
    \end{itemize}
\end{itemize}
\begin{figure}
    \centering
    \includegraphics[width=\figwidth]{age_cdf.pdf}
    \caption{ CDFs of maximum observed drive age (solid) and number of observed drive days within the error log (dashed) for each drive. }
    \label{fig:agecdf}
\end{figure}
For a given drive, the error log may have observations spanning over a period of several days up to several years. This is demonstrated in the ``Max Age'' CDF in Figure~\ref{fig:agecdf}, which shows the distribution over ``oldest" observations we have for each drive. This measure indicates the length of the observational horizons we possess.
\begin{table}
	\centering
    \begin{tabular}{lrrr} \toprule
		Error type & MLC-A & MLC-B & MLC-D \\ \midrule
        {correctable error} & 0.828895 & 0.776308 & 0.767593 \\
        {final read error} & 0.001077 & 0.001805 & 0.001552 \\ 
        {final write error} & 0.000026 & 0.000027 & 0.000034 \\ 
        {meta error} & 0.000014 & 0.000016 & 0.000028 \\
        {read error} & 0.000090 & 0.000103 & 0.000133 \\ 
        {response error} & 0.000001 & 0.000004 & 0.000002 \\ 
        {timeout error} & 0.000009 & 0.000010 & 0.000014 \\ 
        {uncorrectable error} & 0.002176 & 0.002349 & 0.002583 \\ 
        {write error} & 0.000117 & 0.001309 & 0.000162 \\ \bottomrule
        \\
   	\end{tabular}
    \caption{Proportion of drive days that exhibit each error type}
    \label{table:fields}
    % \vspace{-15pt}
\end{table}

We observe that, for over 50\% of drives, we have data extending over a period of 4 to 6 years. However, some of these days of drive activity are not recorded in the log. Accordingly, we may ask what magnitude of data we have access to for a given drive. The accompanying ``Data Count'' CDF shows exactly this: the number of drive days that are recorded in the error log for each drive. ``Data Count" is a measure of the volume of the log entries. Measuring them as a function of time is reasonable as there is one log entry per day per drive. 
The data shown in Figure~\ref{fig:agecdf} clearly shows that there are ample data available, and therefore amenable to the  analysis presented in this paper.



\begin{table*}
    \centering
    \small
    \begin{tabular}{lrrrrrrrrrcc}
    \toprule
    {} &  erase &  final read &  final write &  meta & read & response & timeout &  uncorrect. &  write &  P/E cycle & bad block \\
    \midrule
    erase             &             1.00 %&                  0.21 &                   0.24 &            0.17 &            0.22 &                0.02 &               0.01 &                     0.20 &             0.32 &             0.32 &                        0.38 
    \\
    final read        &             0.21 &                  1.00 %&                   0.12 &            0.19 &            0.20 &                0.06 &               0.12 &                     0.97 &             0.28 &             0.18 &                        0.37 
    \\
    final write       &             0.24 &                  0.12 &                   1.00 %&            0.35 &            0.30 &                0.24 &               0.44 &                     0.06 &             0.13 &            -0.05 &                        0.19 
    \\
    meta              &             0.17 &                  0.19 &                   {\bf 0.35} &            1.00 %&            0.40 &                0.02 &               0.02 &                     0.16 &             0.14 &            -0.02 &                        0.19 
    \\
    read              &             0.22 &                  0.20 &                   0.30 &            {\bf 0.40} &            1.00 &                %0.03 &               0.03 &                     0.15 &             0.25 &             0.03 &                        0.18 
    \\
    response         &             0.02 &                  0.06 &                   0.24 &            0.02 &            0.03 &                1.00 &             %  0.53 &                     0.03 &             0.02 &             0.03 &                        0.01 
    \\
    timeout           &             0.01 &                  0.12 &                   {\bf 0.44} &            0.02 &            0.03 &                {\bf 0.53} &               1.00 &  %                   0.03 &             0.02 &             0.00 &                        0.01 
    \\
    uncorrectable    &             0.20 &                  {\bf 0.97} &                   0.06 &            0.16 &            0.15 &                0.03 &               0.03 &                     1.00 &             %0.28 &             0.19 &                        0.37 
    \\
    write             &             {\bf 0.32} &                  0.28 &                   0.13 &            0.14 &            0.25 &                0.02 &               0.02 &                     0.28 &             1.00 &          %   0.23 &                        0.34 
    \\
    P/E cycle            &             {\bf 0.32} &                  0.18 &                  $-0.05$ &           $-0.02$ &            0.03 &                0.03 &               0.00 &                     0.19 &             0.23 &             1.00                       % 0.16 
    \\
    bad block count &             {\bf 0.38} &                  {\bf 0.37} &                   0.19 &            0.19 &            0.18 &                0.01 &               0.01 &                     {\bf 0.37} &             {\bf 0.34} &             0.16              & 1.00           	\\
    drive age &  0.20 & \textbf{0.36} & 0.06 & 0.05 & 0.06 & 0.04 & 0.05 & \textbf{0.36} & 0.14 & \textbf{0.73} & 0.18 \\
    \bottomrule
    \\
    \end{tabular}
    \caption{Matrix of Spearman correlations among cumulative error counts and cumulative P/E cycle count. Bolded text indicates a large correlation value.}
    \label{tab:correlationmatrix}
\end{table*}


The errors collected in the error log  can be separated into two types: {\em transparent} and {\em non-transparent} errors. Transparent errors (i.e., correctable, read, write, and erase errors) may be hidden from the user while non-transparent errors (i.e., final read, final write, meta, response, timeout, and uncorrectable errors) may not.
Incidence statistics for each of these error types are listed in Table~\ref{table:fields}.
Note that meta, response, and timeout errors  are very rare. Uncorrectable errors  and final read errors are more common at least by one order of magnitude comparing to other errors.
For a detailed analysis of this data set focusing on raw bit error rates, uncorrectable bit error rates, and their relationships with workload, age, and drive wear out, we direct the interested reader to~\cite{BiancaFAST16}. 
    %Final read errors correlate significantly with uncorrectable errors, indicating that they likely describe similar behaviors

SSDs can only experience a finite number of write operations before their cells begin to lose their ability to hold a charge. Hence, manufacturers set a limit to the number of P/E cycles a given drive model can handle. For our drive models, this limit is 3000 cycles.
Due to these limits, it is believed that errors are caused in part by wear of write operations on the drive, which one can measure using either a cumulative P/E cycle count or a cumulative count of write operations. Using either measure is equivalent since they are very highly correlated. 
% However, error counts do not correlate significantly with cumulative P/E cycle count (or equivalently with cumulative write count, as these two measures have a strong relationship). 
%{\bf We need the definition of P/E cycles, where we describe the logs.}

Table~\ref{tab:correlationmatrix} illustrates the Spearman correlation matrix across pairs of all measures, aiming to determine whether there are any strong co-incidence relationships between different error types. Spearman correlations are used as a non-parametric measure of correlation, with values ranging between $-1$ and $+1$. The Spearman correlation differs from the more common Pearson correlation in that it is able to detect all sorts of monotonic relationships, not just linear ones~\cite{statistics}.
In Table~\ref{tab:correlationmatrix}, we are especially interested in {\em non-transparent} errors because they are those that are most indicative of aberrant behavior.
Bolded values are those with magnitude greater than or equal to $0.30$, indicating a non-negligible relationship between the pair.

It is interesting to observe that there is little-to-no correlation of
P/E cycle count with any of the other errors, except for some moderate correlation with erase errors. which contradicts common expectations. One reason for this is the aforementioned argument regarding device wear. Another is that drives which experience more activity will simply have more opportunities for errors to occur. We are unable to detect any substantial effects even due to this na\"\i{}ve relationship.
Note that the correlation value of P/E cycle count and uncorrectable error count (which reflects bad sectors and eventual drive swap) is mostly insignificant. {
The age of a drive gives a similar metric for drive wear, which correlates highly with the P/E cycle count. The drive age also has very small correlation with cumulative error counts, with the exception of uncorrectable/final read errors.
}
Bad blocks, another likely culprit for drive swaps, shows some mild correlation with erase errors, final read errors, and uncorrectable errors. 
The high value of the correlation coefficient of 0.97 between uncorrectable errors and final read errors is not useful as the two errors represent essentially the same event: if a read fails finally, then it is uncorrectable. 
Yet, we see some moderate correlation values between certain pairs of measures that eventually show to be of use for swap prediction within the context of machine learning-based predictors, see Section~\ref{sec:ML}.


\observations{
		\textbf{Observation \#1:} There is no clear relationship between non-transparent error types and uncorrectable error counts that presumably result in bad sectors and eventual drive failures.
		Program--erase (P/E) cycle counts, an indicator of drive wear, show very low correlations with most uncorrectable errors and mild correlation with erase errors (transparent errors). Drive age shows a similar pattern of correlation.
}

\observations{
		\textbf{Observation \#2:} Correlations among all pairs of transparent and non-transparent errors show that some pairs may be mildly correlated and can be useful in prediction. Yet, there is no strong indication as to which measures are most useful for prediction.
}





\section{Drive Swap and Repair}
\label{sec:SSDtraceSwapLog}
% \remove{The second log that we use is the {\em swap log}. This log contains one entry for each time a drive is extracted to be repaired. The log reports the drive's ID number and the timestamp of the extraction.} 
{In addition to daily performance metrics, special ``swap'' events are also reported in the data. These events indicate the time at which failed drives are extracted to be repaired.} 
\newtext{Swaps denote visits to the repairs process --- and not simply a swapping out for storing spare parts, or moving a healthy SSD to a storage cabinet. All swaps follow drive failures, and accordingly, each swap documented in the log corresponds to a single, catastrophic failure.} 
Incidence statistics for these \newtext{swaps/failures} are provided in Table~\ref{table:swapdesc}. 
%The third log is the {\em bad chip log}, which reports when one of a drive's chips are marked as ``bad.'' This is done when a certain number % what proportion?
%of the chip's blocks have experienced a non-transparent error and are removed from use [cite Bianca].
%{\bf E: Do we use the bad chip log?}



\begin{table}
	\centering
	\begin{tabular}{lrr} \toprule
		Model & \#Failures & \%Failed \\ \midrule
        MLC-A & 734 & 6.95 \\
        MLC-B & 1565 & 14.3 \\ 
        MLC-D & 1580 & 12.5 \\
        All   & 3879 & 11.29 \\
        \bottomrule
        \\
	\end{tabular}
    \caption{High-level failure incidence statistics. This includes, for each model, the number of failures observed and the proportion of drives that are observed to fail at least once.}
    \label{table:swapdesc}
\end{table}
\begin{table}[htb]
	\centering
    \begin{tabular}{ccc}
    \toprule
    Number of Failures &  \% of drives &\% of failed drives \\
    \midrule
    0 &  88.71 & ---\\
    1 &  10.10 & 89.60 \\
    2 &  1.038 & 9.208 \\
    3 &  0.133 & 1.180 \\
    4 &  0.001 & 0.001 \\
    \bottomrule \\
    \end{tabular} 
    \caption{Distribution of lifetime failure counts. The distribution is expressed with respect to the entire population of drives and with respect to those drives which fail at least once (``failed drives'').}
    \label{tab:nswappdf}
    % \vspace{-10pt}
\end{table}

\newtext{
 Table~\ref{table:swapdesc} shows that failures occur to a significant proportion of drives and are a relatively common occurrence in this data center: a whole 14.3\% of MLC-B drives have failed at least once, followed by 12.5\% of MLC-D drives and 6.95\% of MLC-A ones. This high frequency of failures/swaps  poses a large pressure in terms of maintenance costs, since each swap requires manual intervention. Table~\ref{tab:nswappdf} provides more insights by providing statistics on the frequency of failures for the {\em same} drive.  Unexpectedly, we find that some drives have failed as many as four times over the course of their lifetime. Nonetheless 89.6\% of drives that have been swapped, are swapped only once. }

% Table~\ref{tab:nswappdf} shows the relative frequencies of different swap counts.
% Google's exact methodology for choosing when to swap a drive is unknown to us.

\newtext{
% One of our goals in this paper is to better understand what drive activity necessitates intervention from the repairs process. 
To better characterize the conditions of failure that lead to these repairs, we must pinpoint the failures in the timeline. A natural way to proceed is to define failure events with respect to swap events: a failure occurs on a drive's last day of {\em operational activity} prior to a swap. This is a natural point of failure since, after this point in the timeline, the drive has ceased normal function and is soon be sent to the repairs process.
}

\newtext{
We now discuss what we consider to be ``operational activity.''
It is often the case (roughly $80\%$ of the time) that swaps are preceded by at least one day for which {\em no performance summaries} are documented in the log. This indicates that the drive was non-operational during this period, having suffered a complete failure. }
Prior to this period, we also find substantially higher rates of inactivity relatively to normal drive operation. In this case, inactivity refers to an absence of read or write operations provisioned to the drive. A period of inactivity like this is experienced prior to 36\% of swaps. The length of these inactive periods is less than one week in a large majority of cases.
The existence of such inactivity is an indication that
% the drive may have already failed and is now unable to operate or that the drive has failed noticeably enough that 
data center maintainers no longer provision workloads onto the drive: this amounts to a ``soft'' removal from production before the drive is physically swapped. Accordingly, we define a failure as happening directly prior to this period of inactivity, if such a period exists. 



To summarize, drive repairs undergo the following sequence of events, represented in Figure~\ref{fig:timeline}: {1) At some point, the drive undergoes a failure, directly after which the drive may cease read/write activity, cease to report performance metrics, or both, in succession.}
2) Data center maintenance takes notice of the failure and swap the faulty drive with an alternate. Such swaps are notated as special events in the data. 3) After a visit to the repairs process, a drive may or may not be returned to the field to resume normal operation. 

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{tl_updated.png}
    \caption{Overview of failure timeline 
    % \remove{NOTE: update figure to add another section for inactive period OR expand non-operational period definition to include no-reads/writes period + no-data period?}
    }
    \label{fig:timeline}
    % \vspace{-10pt}
\end{figure}

\begin{table*}[t]
	\centering
    \begin{tabular}{lrrrrrrr} \toprule
		Model & 10 days  & 30 days  & 100 days  & 1 year & 2 years & 3 years & $\infty$  \\ \midrule
        MLC-A & 3.4 (0.23) & 5.0 (0.34) & 6.1 (0.43) & 17.4 (2.61) & 37.6 (2.61) & 43.6 (3.03) & 53.4 (3.71)\\
        MLC-B & 6.8 (0.98) & 9.4 (1.34) & 12.7 (1.81) & 25.3 (3.62) & 36.1 (5.16) & 42.7 (6.11) & 43.9 (6.28) \\ 
        MLC-D & 4.9 (0.61) & 8.1 (1.01) & 15.8 (1.97) & 28.1 (3.51) & 43.5 (5.44) & 50.2 (6.28) & 57.6 (7.20)\\
        \bottomrule
        \\
	\end{tabular}
    \caption{Percentage of swapped drives that re-enter the workflow within $n$ days. The percentage of repaired drives as a function of all drives is also reported within the parentheses.}
    \label{table:swapreenter}
\end{table*}

We will now characterize each of these three stages, in turn. We start by examining the operational periods observed in the swap log.
Figure~\ref{fig:opperiodcdf} presents the CDF of the length of operational periods (alternately denoted ``time to failure''). The CDF includes both operational periods starting from the beginning of the drive's lifetime and operational periods following a post-swap re-entry. It is interesting to note that more than 80\% of the operational periods are {not observed} to end in failure during the 6 year sampling period; this probability mass is indicated by the bar centered at infinity.  
The figure indicates that there is substantial variability in the drive operational time, with the majority of operating times being long. Yet, there is a non-negligible portion of operating times that are interrupted by  failures.
\begin{figure}
    \centering
    \includegraphics[width=\figwidth]{images/opperiod_cdf.pdf}
    \caption{CDF of the length of the drive's operational period. The bar indicates what proportion of operational periods are not observed to end.}
    \label{fig:opperiodcdf}
\end{figure}

%However, there are several issues with this storyline of drive failure. 
We now turn to the non-operational periods. In Figure~\ref{fig:fsdistcdf}, the CDF of the length of the pre-swap non-operational period is shown, i.e., the elapsed time between  the  drive  failure  and  when  it  is  swapped  out  of production.
One  can  see  that  roughly  20\%  of  failed  drives  are  removed within  a  day  and  roughly  80\%  of  failed  drives   are swapped out of the system within 7 days.
However, this distribution has a very long tail (note the logarithmic scale on the x-axis). A non-negligible proportion of failed drives (roughly 8\%) remain in a failed state for upwards of 100 days before they are removed from production. Since these faulty drives can remain in limbo for upwards of a year, the data suggest that these drives may simply have been forgotten in the system. 
\begin{figure}
	\centering
    \includegraphics[width=\figwidth]{lengthnoop_cdf.pdf}
    \caption{CDF of length of non-operational period preceding a swap. This is the number of days between the swap-inducing failure and the physical swap itself. }
    \label{fig:fsdistcdf}
    % \vspace{-15pt}
\end{figure}

Similarly, we turn to Figure~\ref{fig:ttrccdf} for the CDF of the length of the repairs process, a.k.a.~the ``time to repair.'' 
We find that half of drives are never observed to re-enter the field (i.e., the time to repair is infinite -- their share of probability mass is again indicated by the bar). Furthermore, among drives that \textit{are} returned to the field, a majority of them remain in the repairs process for upwards of a year with a maximum repair time of 4.85 years.
\begin{figure}
 \centering
    % \includegraphics{ttr_ccdf.pdf}
    \includegraphics[width=\figwidth]{ttr_ccdf.pdf}
    \caption{CDF of time to repair, ranging from 1 day to 4.85 years. The proportion of repairs that are not observed to terminate is depicted with the bar graph.} 
    \label{fig:ttrccdf} 
    % \vspace{-10pt}
\end{figure}


Restating the results in Figure~\ref{fig:ttrccdf}, Table~\ref{table:swapreenter} illustrates the percentage of swapped drives that are repaired and re-enter the system after a period of $n$ days in repair, the percentage of the successfully repaired drives as a function of all drives is also shown within  the parentheses. These metrics demonstrate that repairs are very slow and that only half of the swapped drives are eventually returned to production by the end of the 6-year trace period.
% \remove{Since repairs that are longer than a year are probably not viable, we surmise that the ID of these drives have been re-purposed and are given to new drives that are put into production.}
%with such long repair times reflect for all practical purposes new ones that are put into production with a reused ID number.

\observations{
        \textbf{Observation \#3:} Failed drives are often swapped out of production within a week, though a small portion may remain in the system  even longer than a year.
}

\observations{
		\textbf{Observation \#4:} While a significant percentage of drives (up to 14.3\% for MLC-B, slightly smaller percentages for the other MLC types) are swapped during their lifetime, only half of failed drives are seen to successfully complete the repairs process and re-enter the field.
}

\observations{
		\textbf{Observation \#5:} Of those repairs that do complete, only a small percentage of them finish within 10 days. About half of drives that are swapped out are not successfully repaired.
}



% We are interested in finding out what are the potential reasons for swaps. 
% It is natural to presume that  potential reasons for swaps may include the occurrence of a large number of errors or a large bad block count. However, these are insufficient for swap prediction. In fact, {\em 26\% of swaps happen to drives which have previously incurred no non-transparent errors and which have developed no bad blocks.}
% In the following section we show evidence of the above fact. {\bf This paragraph doesn't seem to fit in here? I moved this statistic into Section IV}


% {\bf We need to have some discussion as to understanding what leads to errors and what leads to swaps. To this end, we should present also the activity of the drives read/write/etc.}

\section{Symptoms and Causes of SSD Failures}
\label{sec:data}



% \begin{figure}
% 	\centering
%     \includegraphics[width=0.9\linewidth]{nswap_pdf2.png}
%     \caption{Probability that a drive is swapped $n$ times over the course of its lifetime {\tt replace with table?}}
%     \label{fig:nswappdf}
% \end{figure}

\subsection{Age and Device Wear}
\label{subsec:age}

In this section we make an effort to connect the statistics from the two logs, aiming to identify causes of drive failures.
Recall that Table~\ref{tab:nswappdf} shows that, among the drives represented in the error log, 11.29\% of them are swapped at least once.
A natural question is when do these swaps (and the preceding  failures) occur in the drive's lifetime: what is the role of age in drive failure?
% Trace analysis shows that 
% many of these failures occur early in the drive lifetime.
Figure~\ref{fig:swapagepdf} reports the CDF of the failure age (solid line) as a function of the drive age. The figure shows that there are many more drive failures in the first 90 days of drive operation than at any other point in the drive's lifetime. In fact, 15\% of observed failures occur on drives less than 30 days old and 25\% occur on drives less than 90 days old. This seems to indicate that these drives have an infancy period during which drive mortality rate is particularly high. This performance pattern has been noticed previously in similar studies of SSDs in the wild~\cite{MezaWKM15}.
\begin{figure}
	\centering
%     \includegraphics[width=0.9\linewidth]{swapage_pdf.png}
%     \includegraphics[width=0.9\linewidth]{swapage_cdf.png}
%     \includegraphics{prob_fail.pdf}
    \includegraphics[width=\figwidth]{prob_fail.pdf}
    \caption{The CDF of the age of failed drives (solid line) and the proportion of functioning drives that fail at a given age level, in months (dashed line). 
    }
    \label{fig:swapagepdf} 
     
\end{figure} 

    
The slope of the CDF in Figure~\ref{fig:swapagepdf} gives us an estimate of the rate at which swaps occur at a given drive age. However, this estimate is skewed since not all drive ages are equally represented in the data. For example, the rate of failures seems to slow down following the four year mark, but this is due to the fact that drives of this age level are not as common in the data. We hence normalize the number of swaps within a month by the amount of drives represented in the data at that month to produce an unbiased failure {\em rate} for each month (dashed line in Figure~\ref{fig:swapagepdf}). We see that this rate evens out after the third month, indicating that the length of this observed high-failure infancy period is approximately 90 days. Accordingly, for the remainder of this paper, we distinguish drive swaps as {\em young} versus {\em old}, i.e., those swaps occurring before vs.~after the 90-day mark. Beyond the 90-day mark, we observe that the failure rate is roughly constant, suggesting that, even as drives become very old, they are not any more prone to failure.

\IGNORE{
\begin{figure}
    \centering
    \includegraphics{cue_cdf_failed.pdf}
    \includegraphics{cbb_cdf_failed.pdf}
    \caption{CDF of cumulative uncorrectable error counts at time of failure. CDF of cumulative UE counts for drives that do not experience failure.}
    \label{fig:uecdffailed}
\end{figure}
}

% \begin{figure}
% 	\centering
%     \includegraphics[width=0.9\linewidth]{swapage_pdf_bype.png}
%     \includegraphics[width=0.9\linewidth]{prob_fail_bype.png}
%     \caption{Analogous P/E results}
% \end{figure}
%{\bf REgarding Figure2: is it possible to also plot it as a CDF to see which of the two versions are the best. Also, where is the figure that makes the point about new/old drives?}

\newtext{
One potential explanation for the spike in failures for infant drives is that they are undergoing a ``burn-in'' period. This is a common practice in data centers, wherein new drives are subjected to a series of high-intensity workloads in order to test their resilience and check for manufacturing faults. These increased workloads could stress the drive, leading to a heightened rate of failure. To test this hypothesis, we looked at the intensity of workloads over time. For each month of drive age, we examined drives of that age and how many write operations they processed per day. The distributions of these write intensities are presented in Figure~\ref{fig:writerates}. 
}

\newtext{
It is clear that younger drives do \textit{not} tend to experience more write activity than usual (in fact, they tend to experience markedly \textit{fewer} writes!). A similar trend is apparent for read activity (not pictured). We conclude that there is no burn-in period for these drives and that the spike in failure rates is caused by manufacturing malfunctions not caught by drive testing.
}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{images/writerates.pdf}
    \caption{Quartiles of the daily write intensity per month of drive age. The line plot shows the median write intensity for each month. The 1st and 3rd quartiles are shown as the boundaries of the shaded area.}
    \label{fig:writerates}
\end{figure}

Beyond drive age, we are also interested in the relationship between failure and device wear, which we measure using P/E cycles, as discussed in Section~\ref{sec:SSDtraceErrorLog}. In the same style as Figure~\ref{fig:swapagepdf}, Figure~\ref{fig:swapPEpdf} illustrates 
the relationship of cumulative P/E cycles and probability of failure in the form of a CDF (solid line) and an accompanying failure rate (dashed line).
The CDF illustrates that almost 98\% of failures occur before the drive sees 1500 P/E cycles. This is surprising, considering that the manufacturer guarantees satisfactory drive performance up until 3000 P/E cycles. Conversely, the failure rate beyond the P/E cycle limit is very small and roughly constant. The spikes at 4250 and 5250 P/E cycles are artifactual noise attributed to the fact that the number of drives that fail at these P/E levels are so few in number.
% The spikes in the dashed line illustrate the probability of drive failure/swap at certain P/E values but there is no clear trend, 
%this further corroborates that using a threshold of P/E cycles as an omen of imminent drive swap is not informative.
\begin{figure}
 \centering
    \includegraphics[width=\figwidth]{prob_fail_bype.pdf}
    \caption{The distribution  P/E cycle counts of failed drives (solid) and the proportion of drives that fail (dashed) at a given P/E level, binned in increments of 250 cycles. }
    \label{fig:swapPEpdf} 
\end{figure} 

In the figures discussed, we observe high failures rates for both drives with age less than three months and drive with fewer than 250 P/E cycles. Due to the correlation between age and P/E cycles, these two characterizations may be roughly equivalent, describing the same phenomenon. However, we do not find this to be the case. To illustrate this, we plot two CDFs in Figure~\ref{fig:pecountsplit}: one for young failures and one for old ones. It is clear that the young failures inhabit a distinct, small range of the P/E cycle distribution. Since this range is so small, the individual P/E cycle counts are not informative to young failures.

% if we have a young failure, then the p/e cycle is not informative

\begin{figure}
    \centering
    \includegraphics[width=\figwidth]{images/cdf_pe_count_split.pdf}
    \caption{The CDF in Figure~\ref{fig:swapPEpdf} split across infant failures (occurring at age $\le 90$ days) and mature failures (occurring at age $> 90$ days).}
    \label{fig:pecountsplit}
\end{figure}

\observations{
		\textbf{Observation \#6:} Age plays a crucial role in the SSD failure/swap incidence. In particular, drives younger than 90 days have markedly higher failure incidence rates. {This phenomenon is characteristic to young drives and cannot be explained with P/E cycle counts.}
}

\observations{
		\textbf{Observation \#7:} Beyond the infancy period, age does not seem to have an important part to play in failure rate. The oldest drives seem to fail with roughly the same frequency as young, non-infant drives.
}

\observations{
		\textbf{Observation \#8:} The vast majority of drive failures happen well before the P/E cycle limit is reached. Furthermore, drives operating beyond their P/E cycle limit have very low rates of failure.
}

% As mentioned previously, preceding a swap, there tend to be several days when the drive is non-operational, i.e., there is no recorded activity is recorded in the error log. 
% We define a {\em swap-inducing failure} to be a failure that occurs on the first day of the non-operational period preceding a swap. We refer to swap-inducing failures simply as ``failures.''


% \IGNORE{
% Following a swap, a drive may or may not be used again. For 47\% of swaps, the drive is placed back into production 
% For the remaining drives, we find that the drive is only replaced after a large amount of time has passed. On average, this waiting period is approximately three years long! The distribution of the length of this period is shown in Figure~\ref{fig:swaplengthcdf}. We see that, for some drives, the drive is removed from production for over five years.

% \begin{figure}
% \centering
%   \includegraphics[width=0.8\linewidth]{swaplength_cdf.png}
%     \caption{CDF of swap--reentry distance}
%     \label{fig:swaplengthcdf}
% \end{figure}
% } % end of IGNORE, info provided in Table 3

\subsection{Error Incidence}

Intuitively, we would expect that catastrophic drive failure is preceded by previous lapses in drive function, indicated in our data as non-transparent errors. In particular, we focus on uncorrectable errors and bad blocks since they are by far the most common of these errors. Other errors occur far too rarely to give much insight. We test the validity of our intuition by comparing the cumulative counts of errors seen by failed drives to a baseline of cumulative error counts taken across drives that are not observed to experience failure. We are also particularly interested to see if there is any difference in error incidence between young failures ($\le 90$ days) and old failures ($> 90$ days). This is illustrated with CDFs in Figure~\ref{fig:cfrecdf}. 

% Table~\ref{tab:correlationmatrix} alludes that a relationship may exist between drive lifetime and two metrics: bad block error counts and uncorrectable error counts.
% We show the CDFs of these two metrics as cumulative totals since the beginning of the drive's lifetime.

\begin{figure}
	\centering
    \includegraphics[width=\figwidth]{cbb_cdf_byswapage.pdf}
    \medskip
    \includegraphics[width=\figwidth]{cfre_cdf_byswapage.pdf}
    \caption{CDF of cumulative bad block counts and uncorrectable error counts based on the age at which the swap occurred. The ``Not Failed" CDF corresponds to the distribution over drives that are not observed to fail.}
    \label{fig:cfrecdf}
    % \vspace*{-10pt}
\end{figure}
% Note that we also generated the same graphs for final read error counts. Since these results are very similar to those of final read counts and not reported here due to lack of space.
% The ``Not Failed'' line corresponds to the statistics on drives that do not experience any failure in their operational period. We see that young swaps experience these error types much more frequently than average and much more frequently that for older swaps. 
% It is interesting to note that the healthy drives have much higher counts of both measures, perhaps because of their longevity.

We find that drives that fail tend to have experienced orders of magnitude more uncorrectable errors and bad blocks than we would expect, on average. This is exemplified by the fact that in roughly 80\% of cases, non-failed drives are not observed to have experienced any uncorrectable errors. On the other hand, for failed drives, this proportion is substantially lower: 68\% for young failures and 45\% for old drives. In fact, broadening our scope, we find that 26\% of failures happen to drives which have experienced no non-transparent errors \textit{and} which have developed no bad blocks. Furthermore, we find that, if errors \textit{are} observed, then young failures tend to see more of them than old failures. This is most easily seen in the tail behavior of the aforementioned CDFs; for example, the 90th percentile of the uncorrectable error count distribution is two orders of magnitude larger for young failures than for old failures, in spite of the fact that the young drives have been in operation for much less time.

Overall, the presence of errors is not a very good indicator for drive failure since most failures occur without having seen \textit{any} uncorrectable errors. However, drives that experience failure do have a higher rate of error incidence, which means that we expect error statistics to be of some utility in failure prediction (to be discussed in Section~\ref{sec:ML}). Furthermore, we find that the patterns of error incidence are markedly different among young and old failures. In particular, young failures have a predilection toward extremely high error counts.

Moving into a finer temporal granularity, we are interested in error incidence directly preceding the failure. This behavior is of particular importance for failure forecasting and prediction. We ask: do drives tend to be more error-prone right before a failure occurs? How long before the drive failure  is this behavior noticeable? Figure~\ref{fig:uebeforeswap} shows two relevant uncorrectable error statistics in the period before a drive swap. 
% We select uncorrectable errors as they are strongly related to final read errors (see Table~\ref{tab:correlationmatrix}, the correlation coefficient is 0.97). 

The top graph shows the probability that a faulty drive had an error within the last $N$ days before its failure. The baseline is the probability of seeing an uncorrectable error within an arbitrary $N$-day period. We see that failed drives see uncorrectable errors with a much higher than average probability and that this behavior is most noticeable in the last two days preceding the failure. 
However, the probability that a failed drives does not to see any errors in its last 7 days is very high (about 75\%).

The bottom graph shows the distribution of those uncorrectable error counts that are nonzero on each day preceding the swap. We find that error counts tend to increase as the failure approaches. We also find that young failed drives, if they suffer an error, tend to experience orders of magnitude more errors than older ones, note the log-scale on the y-axis of the graph.

To summarize, we zoom in specifically on the period directly preceding a failure. We show that error incidence rates depend on two factors: (1) the age of the drive (young vs.~mature) and (2) the amount of time until the swap occurs. The resulting increase in error rate is most noticeable in the two days preceding the swap, suggesting that the lookahead window within which we can accurately forecast failure may be small.

\begin{figure}
    \centering
    \includegraphics[width=\figwidth]{images/prob_ue_beforeswap.pdf}
    \includegraphics[width=\figwidth]{images/ue_count_beforeswap.pdf}
    \caption{(Top) Probability of uncorrectable error (UE) happening within the last $n$ days before a swap. The baseline curve on the top graph is the probability of seeing an uncorrectable error within an arbitrary $n$-day period. (Bottom) Provided a UE happens, how many occur? Upper percentiles of the distribution of uncorrectable error counts preceding to failure, excluding zero counts. }
    \label{fig:uebeforeswap}
    % \vspace*{-10pt}
\end{figure}

\observations{
	\textbf{Observation \#9:} Incidence of non-transparent errors is not strongly predictive of catastrophic drive failure. In fact, a substantial proportion of drives experience failure without having ever seen any sort of serious soft error.
}

\observations{
	\textbf{Observation \#10:} Failures of young drives are more likely to have seen higher rates of error incidence than failures of mature drives.
}

\observations{
	\textbf{Observation \#11:} Error incidence rates increase dramatically in the two days preceding a drive failure.
}
	
%   \vspace*{-5pt}


% \subsection{Workloads}
% \label{subsec:workloads}

% \remove{
% Our final consideration is that of workloads. We have already considered cumulative write behavior via our analysis of cumulative P/E cycle counts in Section~\ref{subsec:age}. Another set of features  we found to be of interest are read and write operation counts directly preceding the failure. What we found is that drives that are soon to fail are more likely not to have \textit{any} read or write activity. Figure~\ref{fig:probreadwritebeforeswap} shows this phenomenon for the 30 days preceding a failure relative to a baseline average collected across the whole error log. We see that the probability of having no reads/writes increases as the failure date approaches. In particular, for old drives, the probability jumps sharply in the last two days before the failure (echoing the two-day window we found in Figure~\ref{fig:uebeforeswap}).
% }
% \remove{
% What this potentially tells us is that, for some drives, data center administrators are aware of potential unreliability and are choosing not to provision workloads onto these drives. Regardless of whether this is the case, we find that failures remain largely spurious and difficult to predict. This is evidenced in our discussion of relevant features in this section and will be discussed further in Section~\ref{sec:ML}.
% }

% {\bf maybe we should just delete figure 11? i don't think it fits in anywhere and i'm not sure that it tells us anything that important}
% {\bf E: it does not fit in the characterization. Has interesting behavior but somehow expected. I agree to yank it out.}

% \vspace{0.5cm}
% \hspace{-0.3cm}\fbox{\begin{minipage}{8.5cm}
% 		\remove{\textbf{Observation \#12:} Directly preceding to a failure, drives tend to see reduced workloads.}
% 	\end{minipage}}
%   \vspace{0.3cm}

% \remove{In summary, it is clear that none of the metrics discussed can be used effectively to directly predict when a drive failure will occur. However, we have demonstrated that there are observable differences in the behavior of failure-prone vs.~non-failure-prone drives. In the next section we harness these differences to develop machine learning models that encapsulate most of the metrics in the system logs for prediction.}

% \begin{figure}
%     \centering
%     \includegraphics{images/prob_read_beforeswap.pdf}
%     \includegraphics{images/prob_write_beforeswap.pdf}
%     \caption{
%     \remove{
%     Probability that the drive has zero reads/writes on each day prior to the swap. This probability is not cumulative like in Figure~\ref{fig:uebeforeswap}. Baseline probabilities are the probability of zero activity on an arbitrary day for an arbitrary young/old drive.
%     }
%     }
% \label{fig:probreadwritebeforeswap}
% \end{figure}

% \begin{figure}
%     \centering
%     % \includegraphics{images/post_reentry_reads_log_long.pdf}
%     % \includegraphics{images/post_reentry_reads_overlay.pdf}
    
%     \includegraphics{images/post_reentry_reads2.pdf}
%     \includegraphics{images/post_reentry_reads.pdf}
    
%     \caption{Re-provisioning of workloads after drive re-entry. Whiskers signify 10th and 90th percentiles. Drive workloads seem to stabilize after a week of activity. ``Baseline'' is the distribution of daily read counts over the whole error log. The baseline probability in the top graph is represented with a horizontal dashed line.}
%     \label{fig:reentrystats}
% \end{figure}

\section{Failure Prediction}
\label{sec:ML}

In order to shed light on the causes for failures, we have developed prediction models for the detection of swap-inducing failures. The models predict whether a failure will occur within the next $N$ days for some $N \ge 1$. 

The use case of prediction is clear: if we are able to detect future failures far enough in advance with sufficient certainty, we have the option to take preventative action to mitigate the risk of data loss and downtime. For example, this may involve backing up the faulty drive's data to another disk to act as a spare.

\newtext{That being said, our goal in this section is not simply predictive accuracy. 
% We are \textit{also} concerned with predictive performance as an indicator of a classifier's ability to accurately model the data. 
The machine learning classifiers we consider are simple yet powerful enough to facilitate interpretation and a more thorough investigation into the symptoms and causes of drive failure. For these classifiers, high predictive performance not only indicates the utility of the classifier in a predictive setting, but also its ability to model the log data. Accordingly, high model performance inspires trust in the inferences we draw from the model.
}

\subsection{Model Description and Metrics}
As {\bf input}, we use each of the workload and error statistics itemized in Section~\ref{sec:SSDtraceErrorLog}. For each of these statistics, we include two values: the value of the statistic on the day of prediction as well as a cumulative count over the course of the drive's lifetime. Daily measures are used to provide information about current drive behavior while cumulative measures are used as they readily summarize all previous activity from across the drive's lifetime. \newtext{For example, for each date of prediction, we include both the number of write operations performed by the drive on that day as well as the cumulative number of write operations performed, from the beginning of the drive's lifetime up to the date of prediction.}

The {\bf output} of the models that we consider is a continuous output in the interval $[0, 1]$, which may be interpreted as the conditional probability of failure given the input. \newtext{We often find it useful or necessary to have a binary prediction, i.e., failure vs.~non-failure. Such binary predictions are of great practical importance. To accomplish this,} we may discretize this output into a binary prediction using a discrimination threshold $\alpha$: if the failure probability exceeds $\alpha$, we predict that failure will occur, otherwise we predict that no failure will occur.

%The ROC AUC metric (area under the curve) is used to assess prediction performance~\cite{FAWCETT2006861}
% We utilize on the ROC AUC metric~\cite{FAWCETT2006861} to measure classifier performance due to its robustness in imbalanced problems.
Consistent with the standard practice of evaluating a classifier with highly imbalanced data sets (as is the case here, our data contains 1 failure for each 10,000 non-failure cases), 
we choose to measure predictive performance using the receiver operating characteristic (ROC) curve~\cite{FAWCETT2006861} because it is insensitive to class imbalance. Furtheremore, the ROC curve illustrates the practical, diagnostic performance of a binary classifier as the discrimination threshold $\alpha$ is varied.
The ROC curve plots the true positive rate (i.e.,~recall) against the false positive rate for the selected classifier. 
These are calculated as
\begin{align*}
\mathrm{TPR} & = \frac{\#\text{ of True Positives}}{\#\text{ of Positive Samples}} \\
\mathrm{FPR} & = \frac{\#\text{ of False Positives}}{\#\text{ of Negative Samples}} 
\end{align*}
The values of these two statistics vary depending on the chosen discrimination threshold $\alpha$. Plotting a curve across all values of these two statistics, we find the area under this curve to obtain a summary statistic of classifier performance. This is called the ROC AUC (area under curve) statistic.
The ROC AUC ranges between 0.5 (indicating performance not exceeding that of random guessing) and 1.0 (indicating perfect, deterministic prediction). We chose this metric since it is known to be robust in cases of imbalanced classes~\cite{FAWCETT2006861}.
This is due to the fact that the true positive rate and false positive rate metrics are independent of the level of imbalance.
The false negative rate for the classifier may also be read from the ROC curve using the identity $\mathrm{FNR} = 1 - \mathrm{TPR}$. This transformation allows a method of comparison between our predictions and those shown in a previous machine learning prediction study on this same data set that focuses on predicting the occurence of soft errors only~\cite{mahdisoltani2017proactive}.

\begin{table*}
\centering
\begin{tabular}{lcccc} \toprule
$N$ (lookahead days) & 1 & 2 & 3 & 7 \\ \midrule
Logistic Reg. & $0.796 \pm 0.010$ & $0.765 \pm 0.009$ & $0.745 \pm 0.007$ & $0.713 \pm 0.010$ \\
$k$-NN & $0.816 \pm 0.013$ & $0.791 \pm 0.009$ & $0.772 \pm 0.008$ & $0.716 \pm 0.008$ \\
SVM & $0.821 \pm 0.014$ & $0.795 \pm 0.011$ & $0.778 \pm 0.011$ & $0.728 \pm 0.011$ \\
Neural Network & $0.857 \pm 0.007$ & $0.828 \pm 0.004$ & $0.803 \pm 0.009$ & $0.770 \pm 0.008$ \\
Decision Tree & $0.872 \pm 0.007$ & $0.840 \pm 0.007$ & $0.819 \pm 0.005$ & $0.780 \pm 0.006$ \\
Random Forest & $\mathbf{0.905 \pm 0.008}$ & $\mathbf{0.859 \pm 0.007}$ & $\mathbf{0.839 \pm 0.006}$ & $\mathbf{0.803 \pm 0.008}$ \\
\bottomrule \\
\end{tabular}
\caption{ROC AUC for each prediction model and lookahead window $N$ (in days). The cross-validated mean is presented with the standard deviation across folds. The AUC value of the best model is bolded.}
\label{tab:AUCresults}
% \vspace*{-10pt}
\end{table*}



For further assurance of model validity, 5-fold cross-va\-li\-da\-tion is used. This is done by splitting the drive ID numbers into five equally sized groups. We train the model five times, successively using a different group as the testing set, with the remaining four groups used as the training set. For each train--test split, we calculate the ROC AUC value, and we report the mean value of the metric across the five splits. We found cross-validation to be important since the sampling bias for train--test split can be quite significant in this imbalanced classification problem. Furthermore, error and workload for a given drive are highly correlated across different drive days, leading to results that are biased to be larger than expected. Accordingly, we avoid splitting observations for a given drive across the training and testing sets. This is done by partitioning the folds based on drive ID.

Since we are dealing with a heavily imbalanced data set (out of 40,000,000 observed days of data, we have only 4000 failures), we randomly downsample the majority class to produce a 1:1 positive--negative ratio. This is a standard machine learning tactic used to make the classifier more sensitive to the minority class~\cite{he2008learning}. 
\newtext{One concern with downsampling is that the model is not able to capture all of the variation within the majority class. To ensure the model's accuracy, we performed multiple random downsamplings on the same training set and observed the ROC AUC for each resulting model. We found that the AUC score only wavers on the order of $\pm 0.001$. We determined this variability induced by downsampling to be negligible. We also tested different downsampling ratios beyond 1:1 and observed either miniscule improvements or overall reductions in performance.}


\subsection{Prediction Accuracy}
Table~\ref{tab:AUCresults} reports on the average ROC AUC values for six machine learning predictors: logistic regression, $k$-nearest neighbors ($k$-NN), support vector machine (SVM), neural network, decision tree, and random forest~\cite{alpaydin2014introduction}.
\newtext{For each method, we performed a grid search over hyperparameters in order to find the best configuration. Most of these hyperparameters were regularization parameters, tuning the complexity of the trained model. These include the ridge regression coefficient for logistic regression, the maximum depth of the trees in the random forest, and the sizes of the hidden layers in the neural network. We avoided overfitting by choosing the values of the hyperparameters that provided the best cross-validated performance with respect to ROC AUC.}
The classifiers (and respective AUC predictions) are for the entire log, i.e., we do not distinguish among drive types.
Similarly to~\cite{mahdisoltani2017proactive} where predictions of the disk error types is done (and not the catastrophic failures that we focus on here), we find that Random Forest models perform best on this data set compared to other common classifiers, including logistic regression and neural networks. We believe random forests to be so successful on this data set since they work well with discrete data are able to model nonlinear effects. It is also interesting to see that a single decision tree is able to achieve competitive performance to the random forest ensemble.
In addition, across all models, it is clear that the shorter the lookahead window, the higher the quality of predictions we are able to achieve.

The performance of the Random Forest model is shown for a wider range of values for the detection window size $N$ in Figure~\ref{fig:roccurvebydays}.
We see that for lookahead that ranges up to 30 days, the effectiveness of prediction drops from 0.90 (1 day) to 0.77 (30 days), suggesting that strong prediction of swaps can be done with a range of  windows but predictions are especially strong for 1 to 3 days lookahead.



\begin{figure}
\centering
\includegraphics[width=\figwidth]{lookahead2.pdf}
\caption{Random forest performance as a function of lookahead window size $N$. Error bars indicate the standard deviation of the cross-validated error across folds.}
\label{fig:roccurvebydays}
% \vspace{-10pt}
\end{figure}

Next, we consider the effectiveness of the classifier when evaluated individually on each drive type: MLC-A, MLC-B, and MLC-D. 
Figure~\ref{fig:roccurvebymodel} reports results on this for a 1-day lookahead window and show that the Random Forest model performs nearly identically across the three MLC logs.
Next, to test robustness across MLC model types, we see whether predictive success on one model implies predictive success on another. To test this, we train the classifier using one MLC model in order to predict failures for another.
Table~\ref{tab:RFcrossvalidationMLC} presents the ROC AUC results and shows that this is feasible with AUC values showing only minor degradation. 
Yet, if all data (all three MLC logs) are used for training (see the last column of Table~\ref{tab:RFcrossvalidationMLC}), prediction is superior.

\begin{figure}
\centering
% \includegraphics{roc_bymodel_withauc.pdf}
\includegraphics[width=\figwidth]{roc_bymodel_withauc2.pdf}
% \includegraphics[width=0.9\linewidth]{fprfnr_bymodel.png}
\caption{ROC curves for each drive model with a random forest prediction model and lookahead of $N = 1$ day.}
\label{fig:roccurvebymodel}
\end{figure}



\begin{table}
\centering 
\begin{tabular}{lcccc} \toprule
& \multicolumn{4}{c}{Training model(s)} \\
Test model & MLC-A & MLC-B & MLC-D & All \\ \midrule
MLC-A & {\em 0.891} & 0.871 & 0.887 & {\em 0.901} \\
MLC-B & 0.832 & {\em 0.892} & 0.849 & {\em 0.893} \\
MLC-D & 0.868 & 0.857 & {\em 0.897} & {\em 0.901} \\
\bottomrule \\
\end{tabular}
\caption{Random forest for $N = 1$. Italics indicate that the AUC was estimated with cross-validation.}
\label{tab:RFcrossvalidationMLC}
% \vspace{-10pt}
\end{table}


% \begin{figure}
% \includegraphics{predquality_byage.pdf} 
% \caption{Random forest performance for $N = 1$ as a function of the age of the input {\tt figure out something better}}
% \label{fig:tprfprbyage}
% \end{figure}

% \begin{figure}
% \includegraphics{predquality_bype.pdf}
% \caption{Random forest performance for $N = 1$ as a function of the P/E cycle count of the input}
% \label{fig:tprfprbpe}
% \end{figure}

\subsection{Model Improvement: Using Drive Age}
Recall from the previous section that we found that a large proportion of failures comes from infant drives (i.e., those less than 90 days old, labeled in our discussion as ``young"). We may ask: are there differences in how the model detects infant failures versus mature failures? To see this, we evaluated model performance for each month of drive age. Since the random forest model outputs a prediction probability, to get a binary prediction, we threshold this output. A conservative threshold (i.e., a threshold close to 1) is practical for many real-world prediction applications since a low false positive rate is generally required. Using these binary predictions, we evaluated the true positive rate (i.e.,~recall) on the test set as a function of the age of the input drive. These rate estimates were 5-fold cross-validated and the mean $\mathrm{TPR}$ is reported. The resulting figure is shown in Figure~\ref{fig:tprbyage}. Three reasonable choices of probability thresholds are reported.
We see that, for all three thresholds, the model is able to achieve significantly higher $\mathrm{TPR}$ for drives less than three months old. This is an indication that there are some aspects of infant failures which are more easily detected by the model, leading to superior performance during this period.


\begin{figure}
\centering
% \includegraphics{tpr_byage_diffthreshes.pdf}
\includegraphics[width=\figwidth]{tpr_byage_diffthreshes2.pdf}
\caption{True positive rate as a function of drive ages. Three different prediction thresholds are reported.}
\label{fig:tprbyage}
% \vspace{-10pt}
\end{figure}

To further validate this distinction in predictive performance, we draw separate ROC curves for young and old drive inputs, much like we did for model type in Figure~\ref{fig:roccurvebymodel}. This is shown in Figure~\ref{fig:roccurvebyage}. We confirm that the performance on young drives is consistently better than on older drives, as evidenced by the superior AUC score. To obtain even better performance, we chose to partition the data set completely into infant and mature age groups and train these two subsets separately.
% This is significant because a large proportion (20\%) of swap-inducing failures are infant failures.
% To this end, we split the data set into two parts: infant drive data and mature drive data. 
% We run our failure detection algorithm on both of these subsets. 
% {\bf E: Should we make the fact that young drive failures are fundamentally more predictable than others an observation???}
We find that infant drive classifier has a ROC AUC value of \newtext{$\mathbf{0.970 \pm 0.005}$} while the classifier for older drives has an AUC that is only \newtext{$\mathbf{0.890 \pm 0.005}$}. Thus, young drive failures are fundamentally \textit{more predictable} than those of older drives. This is significant because a large proportion (20\%) of swap-inducing failures are young failures. We conclude that the indications of young drive failure must be more robust than---and fundamentally distinct from---the indications of mature drive failure. This result echoes our characterization of young and old failures discussed in Section~\ref{sec:data}.

\begin{figure}
\centering
% \includegraphics{roc_byage_withauc.pdf}
\includegraphics[width=\figwidth]{roc_byage_withauc2.pdf}
\caption{ROC curves for young (age at most 90 days) versus old (age more than 90 days) drives.  Prediction model is random forest with lookahead $N = 1$ days.}
\label{fig:roccurvebyage}
% \vspace*{-10pt}
\end{figure}

%{\tt what's the effect on the P/E cycle hump (\~{}1000 P/E cycles)?}
\subsection{Model Interpretability}
\label{sec:interp}

The prediction results are respectable for such an imbalanced situation, but one of the great strengths of the Random Forest model is its interpretability. A trained Random Forest model can produce a ranking of input features based on what proportion of variance in the training set they are able to explain. The top features for the models for infant and mature drives are given in Figure~\ref{fig:featureimportance}.
It is interesting to observe that the relative feature importance ranking across the two classifiers is indeed quite different.
For infant drives, the age of drive is the most important one, followed by non-transparent errors: {\em cumulative} values of bad block counts, final read errors, read error counts, and uncorrectable error counts all have importance higher than than 0.08\%.
For mature drives, the features that are most useful for model prediction are instead those that relate to drive wear-and-tear, i.e., read counts, correctable error counts, and write counts, with the cumulative bad block count ranking as the fourth most important feature (for infant drives it is the most important feature).
It is expected that read and write counts are important for failure prediction, given that a drive is more likely to  not have any activity before a failure.
So we conclude that the age and usage of the drive is a very important feature for model prediction accuracy.


\newtext{The prediction scheme we discuss here bears similarity to previous results for this data set, which predicted uncorrectable error incidence~\cite{mahdisoltani2017proactive}. Although we are predicting swap-inducing failures, our methodologies here are extensible to be able to improve the predictions of errors given in~\cite{mahdisoltani2017proactive}.} For example, by partitioning the data into young and old sections, we are able to achieve ROC AUC scores of \newtext{$0.960 \pm 0.009$} and \newtext{$0.931 \pm 0.007$}, respectively. This leads to improved performance when compared to the AUC score of \newtext{$0.933 \pm 0.006$} obtained when training on unpartitioned data. We see this same pattern for the prediction of a variety of non-transparent errors in Table~\ref{tab:nontransparenterrors}. 

\observations{
		\textbf{Observation \#12:} The features that are most important for prediction are very different between young and old failures. In particular, young failures are dominated by age and non-transparent errors, while old failures are more related with drive wear-and-tear.
}

\observations{
		\textbf{Observation \#13:} Infant drive failures are more easily predicted than mature drive failures, indicating that the symptoms are infant drive failures are more robust. This trend holds when predicting a variety of non-transparent errors, as well. Training separate models leads to a substantial boost in predictive performance for young failures.
}
  

\begin{figure}
% \includegraphics{N_1_imps.pdf}
\centering
\includegraphics[width=\figwidth]{N_1_imps2.pdf}
\caption{
Feature importance for the random forest models for infant drives (top figure) and mature drives (bottom).
% {\tt E2J: can you replot the bottom one with x-axis up to .20 so it is easier to compare? Also, replace "ce rate" with "correctable error rate" -- in both graphs.}
}
\label{fig:featureimportance}
\end{figure}

\begin{table}
\centering
\begin{tabular}{lccc} \toprule
Error & Combined & Young & Old \\ \midrule
Bad block & 0.877 & 0.878 & 0.873 \\ 
Erase & 0.889 & 0.934 & 0.882 \\ 
Final read & 0.906 & 0.959 & 0.852 \\
Final write & 0.841 & 0.937 & 0.780 \\
Meta & 0.854 & 0.890 & 0.842 \\
Read & 0.971 & 0.917 & 0.973 \\
Response & 0.806 & --- & --- \\
Timeout & 0.755 & 0.812 & 0.735 \\
Uncorrectable & 0.933 & 0.960 & 0.931 \\
Write & 0.916 & 0.911 & 0.914 \\
\bottomrule \\
\end{tabular}
\caption{ROC AUCs for random forest to predict various error types for $N = 2$. Response errors are too rare to predict for different age granularities. }
\label{tab:nontransparenterrors}
% \vspace{-10pt}
\end{table}

\IGNORE{ -- TO RECONSIDER
To further elaborate on the importance of drive age for error prediction, we used the above definition of young/old and apply it for improving the prediction accuracy of models for uncorrectable errors.
The authors in~\cite{mahdisoltani2017proactive} use the same logs to predict non-transparent errors (not swaps) and conclude that random forests are strong predictors.
Here, we show that we can improve the prediction of errors by training two distinct random forests, one for young drives and one for old ones.
Results are reported in Table~\ref{tab:nontransparenterrors}.
With the split, we find that model performance is greatly improved for certain error types. This gives additional evidence to our conclusion that failure characteristics for infant drives are distinct from older drives, therefore prediction effectiveness benefit greatly from training separate models for young and old drives.

\begin{table}
\centering
\begin{tabular}{lccc} \toprule
Error & Combined & Young & Old \\ \midrule
Bad block & 0.877 & 0.878 & 0.873 \\ 
Erase & 0.889 & 0.934 & 0.882 \\ 
Final read & 0.906 & 0.959 & 0.852 \\
Final write & 0.841 & 0.937 & 0.780 \\
Meta & 0.854 & 0.890 & 0.842 \\
Read & 0.971 & 0.917 & 0.973 \\
Response & 0.806 & --- & --- \\
Timeout & 0.755 & 0.812 & 0.735 \\
Uncorrectable & 0.933 & 0.960 & 0.931 \\
Write & 0.916 & 0.911 & 0.914 \\
\bottomrule \\
\end{tabular}
\caption{ROC AUCs for random forest with $N = 2$. Response errors are too rare to predict for different age granularities. }
\label{tab:nontransparenterrors}
\end{table}

\IGNORE{
Overall, the prediction results are respectable for such an imbalanced situation, but one of the great strengths of the Random Forest model is its interpretability. A trained Random Forest model can produce a ranking of input features based on what amount of variance in the training set they are able to explain. The top features for $N = 2$ are given in Figure\ldots. {\tt insert discussion of most important features}

\begin{figure}
\includegraphics{N_1_imps_monthly_0.pdf}
\includegraphics{N_1_imps_monthly_1.pdf}
\includegraphics{N_1_imps_monthly_2.pdf}
\caption{Importance rankings for models trained on one of each of the first three months of data.}
\end{figure}

\begin{figure}
\includegraphics{auc_byage.pdf}
\caption{{\tt This is here for reference. This is simply the ROC AUC for each month. This was my original direction for trying to show the young--old prediction differences, but as you can see, there are no interesting patterns!}}
\end{figure}
}  % end of IGNORE

\section{To Do:}
\begin{itemize}
\item Could you try to rerun the prediction models to argue for drive backup before swap (if predicted) vs reconstruction?

\item I was also thinking to show drive activity immediately after it is reinstated (after the swap) -- how does the workload change from the overall reads/writes after the drive is reinstated? Essentially this should be the reconstruction?
\end{itemize}
}  % IGNORE


\input{hdd_characterization}


\section{Related Work}
\label{SEC:related}
Large-scale data centers from major service prividers are extensively used to serve millions of jobs on a daily basis~\cite{verma2015large,gill2011understanding,wang2010impact}.
Consequently, reliability of such systems is of great importance.
Much prior work has investigated and analyzed the impact of failures and errors on large-scale data centers~\cite{guo2015pingmesh, wang2017can, schroeder2017reliability, nie2018dsn, ma2015raidshield}.
The storage system hierarchy has been singled out as especially important for reliability, especially for DRAM and HDD failures~\cite{schroeder2007disk, schroeder2009dram, hwang2012cosmic}.
\newtext{
In particular, the other large-scale reliability study of SSDs coming from Facebook~\cite{MezaWKM15} focuses more on hardware-level events. We echo some of their conclusions regarding infant failures in this paper.
}

In order to initiate proactive actions (e.g., drive replacement) before the failure occurs, many works focus on predicting system failures~\cite{hamerly2001bayesian, pinheiro2007failure, ma2015raidshield}.
Hamerly et al.~\cite{hamerly2001bayesian} use Bayesian approaches while Ma et al.~\cite{ma2015raidshield} simply use threshold-based prediction.
Machine learning based failure prediction shows more advantages than heuristics and statistical models. 
%~\cite{xue2016managing}.
{Mahdisoltani et al.~\cite{mahdisoltani2017proactive} explore different machine learning models to predict uncorrectable errors and bad blocks in hard disk drives and solid state disks.}
Ding et al.~\cite{ding2018online} capture the fuzzy rules and combine time series models to predict online software system failures.
Botezatu et. al.~\cite{DorotheaKDD16} and Narayanan et. al.~\cite{NarayananWJSCSC16} use machine learning to predict disk replacements using SMART data.
Xu et. al.~\cite{XuATC18} use SMART data and system-level signals to develop a machine learning model to improve service availability of Microsoft Azure. 

Compared with statistical models in prior works~\cite{hamerly2001bayesian, pinheiro2007failure, ma2015raidshield}, our work leverages machine learning models to predict disk drive failures with low false positive rate.
In contract to prediction for systems in a manufacturer-controlled environment~\cite{murray2005machine} or using data sets of very limited size~\cite{goldszmidt2012finding}, we focus here on trace data collected in a production system consisting of over 10,000 drives over a period of six years.
\newtext{The same trace has been examined in~\cite{mahdisoltani2017proactive} but focused on machine learning models for predicting SSD errors rather than complete disk failures. We recreate and expand their work here in Section~\ref{sec:interp}. Schroeder et al.~\cite{BiancaFAST16} also utilized the same trace, but focused orthogonally on bit error rates, without discussing causes, symptoms, or prediction.}


\section{Conclusion}
\label{sec:conclusion}
In this paper we do a detailed workload characterization study of SSD failures using a Google trace of more than 30,000 drives within a time period of six years in production data centers. We reach several surprising conclusions, in particular, that the usual suspects of drive failure (write behavior and error incidence) are nowhere near as informative as one would expect.
We extract informative features from this characterization to train several machine learning predictors, and find that random forests are the most successful, achieving extremely accurate predictions of drive failure. Our analysis concludes that the age of the drive is a crucial factor for failure prediction. If the drive does not fail within its first 3 months of operation, then wear and tear play a more substantial role in its reliability.
We are currently working on advancing our understanding of disk activity  prior to a swap and directly following re-entry in order to improve our prediction models for large $N$.

% \ifCLASSOPTIONcompsoc
%   % The Computer Society usually uses the plural form
%   \section*{Acknowledgments}
% \else
%   % regular IEEE prefers the singular form
%   % \section*{Acknowledgment}
% \fi

\section*{Acknowledgment}
We deeply thank Arif Merchant of Google for making the SSD trace available to us.
The authors would also like to thank the anonymous reviewers for their comments and suggestions.
This material is based upon work supported by the National 
Science Foundation (NSF) grants (\#1717532 and \#CCF-1649087). 
This work 
was performed in part using computing facilities at the College 
of William \&{} Mary which were provided by contributions from 
the NSF and the Commonwealth of Virginia Equipment 
Trust Fund.
 
\IGNORE{
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{pdp.png}
    \caption{Partial Dependence Plot for Gradient Boosted model. The partial dependence measures the marginal effect of a given variable; higher PD for a value of a predictor indicates that the value is more indicative of failure, on average.}
    \label{fig:pdp}
\end{figure}
}


==> outline.tex <==
\begin{enumerate}
    \item Introduction
    \item Drives characterization
    \begin{enumerate}
        \item For SSDs, observations in Section 2 (SC19)
        \item For HDDs, a similar analysis to the one for SSDs. \textbf{In this case, we considered only the top-5 HDDs, i.e., the five models with more entries}. Main differences:
        \begin{itemize}
            \item differentlu from SSDs, more than 90\% of HDDs is not repaired
            \item HDDs have a shorter life than SSDs
        \end{itemize}
    \end{enumerate}
    \item Causes of failures
    \begin{enumerate}
        \item For SSDs, analysis in Section 4 (SC19)
        \item For HDDs, we can show that drive age does no affect the dependability of an HDD as much as it affects SSDs. Then, we can look into other SMART features that seem to affect the HDD dependability (e.g., smart5, smart192, smart193, smart240).
    \end{enumerate}
    \item Failure prediction
    \begin{enumerate}
        \item We can use a random forest since it has been shown to be efficient for both SSDs (SC19) and HDDs (ATC17, Schroeder -- there, they used it only to predict errors, not failures).
        \item We show that for HDDs and SSDs, the random forest works better when N (i.e., the number of days before failure) is smaller. Moreover, the AUC is larger when we use the HDD dataset.
        \item The AUC depends on the training set. Although for SSDs the AUC is always larger than 0.8, when considering HDDs the AUC goes from 0.65 to 0.9 depending on the considered model. When we train the model on DM001, we obtain the worst result. \textbf{We must choose if we should discard this model or not}. So much different results may mean that each different HDD have different features and failure symptoms.
        \item When considering the recall as a function of drive age:
        \begin{itemize}
            \item for SSDs, Fig. 14
            \item for HDDs, it is initially low, then it increases. Besides drive age, we could also consider other smart features.
        \end{itemize}
        \item The model performance is analyzed by splitting the dataset in two groups (e.g., young and old):
        \begin{itemize}
            \item for SSDs, same analysis as in Section 5.3 (SC19)
            \item for HDDs, we repeat the analysis in Figs. 15 and 16 (SC19) for drive age and other smart features:
                    \begin{itemize}
                        \item Once again, we can show the splitting the dataset in young/old drives does not improve the model performance
                        \item Then, we split the dataset using other features and thresholds and see how the model change
                    \end{itemize}
        \end{itemize}
    \end{enumerate}
    \item Related work
    \item Conclusion
\end{enumerate}
